Functional Stability of Discounted Markov Decision Processes Using Economic MPC Dissipativity Theory

This paper discusses the functional stability of closed-loop Markov Chains under optimal policies resulting from a discounted optimality criterion, forming Markov Decision Processes (MDPs). We investigate the stability of MDPs in the sense of probability measures (densities) underlying the state distributions and extend the dissipativity theory of Economic Model Predictive Control in order to characterize the MDP stability. This theory requires a so-called storage function satisfying a dissipativity inequality. In the probability measures space and for the discounted setting, we introduce new dissipativity conditions ensuring the MDP stability. We then use finite-horizon optimal control problems in order to generate valid storage functionals. In practice, we propose to use Q-learning to compute the storage functionals.

==> additional.tex <==
%The paper is structured as follows. Section \ref{sec:PS} describes the problem setting and formulates MDPs in the density space. We introduce optimal value functional and optimal steady measure in this section. Section \ref{sec:stability} details the functional stability concept and FSDSD conditions for MDPs. In this section, we show that a closed-loop Markov chain is functional stable under the optimal policy if the associated MDP satisfies FSDSD conditions. Section \ref{sec:FA} a introduces functional approximator for the optimal action-value function, which delivers a valid storage function for rich enough parameterization. Section \ref{sec:Conc} delivers the conclusions.
%Section \ref{sec:NS} provides numerical simulation results, and  


For the discounted setting the stage cost \eqref{eq:TL} reads:
\begin{align}
  &L(\vect s,\vect a)=\\ &\left\{\begin{matrix}
 Q^\star(\vect s,\vect a)- V^\star(\vect f(\vect s,\vect a)) & \mathrm{If}\, \left|V^\star(\vect f(\vect s,\vect a))\right|<\infty \\ \infty
 & \mathrm{Otherwise}
\end{matrix}\right.\nonumber
\end{align}
then if there exists a storage function $\lambda$:
\begin{align}
    \lambda (\vect f(\vect s,\vect a)) - \lambda (\vect s) \leq -\rho(\|\vect s\|)+ Q^\star(\vect s,\vect a)- V^\star(\vect f(\vect s,\vect a))
\end{align}
then MPC is dissipative. If the model is same as the real system, then this condition is exactly the second condition of SDSD. Then we can write:
\begin{align}
 V^\star(\vect s)=-\lambda(\vect s)+\min_{\vect\pi}   V^\star(\hat{\vect s}_N)+\sum_{k=0}^{N-1} \bar L(\hat {\vect s}_k,\vect { \pi}\left(\hat {\vect s}_k\right)),\,\, \hat {\vect s}_0=\vect s,
\end{align}
where 
\begin{align}
    &\rho(\|\vect s\|)\leq \bar L(\vect s,\vect a)=:\\ &Q^\star(\vect s,\vect a)- V^\star(\vect f(\vect s,\vect a))+\lambda (\vect s)-\lambda (\vect f(\vect s,\vect a))\nonumber
\end{align}


\section{Functional Dissipativity \& Learning}
We won't have enough time to propose something ``solid", but some reflections to pave the way to what we could say soon would be meaningful. Here are a few thoughts:
\begin{itemize}
    \item We can make the argument for ``learning under the dissipativity constraints" rather than ``verifying the dissipativity constraints" (similar to other papers). In that context, we learn an MPC with a functional stage cost satisfying (6), where the storage function acts as an ``extra degree of freedom" to achieve Q-learning. We may have to admit that the undiscounted case (reverting to the original functional dissipativity) is easier to treat.
\item We could unpack a bit what Q-learning looks like in the functional case. Generally speaking it would be something of the kind:
\begin{align}
    \min_{\vect\theta}\, \mathbb E\left[Q_{\vect\theta}[\delta_{\vect s},\vect a] - Q^\star(\vect s,\vect a)\right]^2
\end{align}
where $\delta_{\vect s}$ is a Dirac measure taken at $\vect s$ and $\mathbb E$ is an expected value over the real state transitions and the exploration (we don't have much of a choice here). What does it imply? 
\item We could add the ``cost modification" story here for the functional case, and then argue that the functional MPC does not need to use a perfect model (and/or could even be deterministic). 
\end{itemize}

Next lemma states the monotonicity property of functional ${\Psi}_{\vect\theta}^{N}$ with respect to the horizon length $N$.
\begin{Lemma} Suppose that \eqref{eq:ter:assum} holds. Then:
\begin{align}\label{eq:mono}
    {\Psi}^{N+1}_{\vect\theta}[\rho_0]\leq {\Psi}^{N}_{\vect\theta}[\rho_0], \quad \forall N\in\mathbb{I}_{\geq 0}
\end{align}

\end{Lemma}
\begin{proof}
For $N=0$, from \eqref{eq:ter:assum}, we have:
\begin{align}
   V^1_{\vect\theta}[\rho_0]&=\min_{\vect\pi}{-\lambda_{\vect\theta}[\rho_0]+T_{\vect\theta}[\rho^{\vect\pi}_1]+\mathcal{L}_{\vect\theta}[\rho_0,\vect\pi]}\nonumber\\&\leq -\lambda_{\vect\theta}[\rho_0]+T_{\vect\theta}[\rho_0]:=V^0_{\vect\theta}[\rho_0]
\end{align}
where $\rho^{\vect\pi}_1\in\Xi_{\mathrm{f}}$. Suppose that for some $N\geq0$, \eqref{eq:mono} holds, then for $N+1$ we have:
\begin{align}\label{eq:pro1}
     V^{N+2}_{\vect\theta}[\rho_0]-&V^{N+1}_{\vect\theta}[\rho_0]= \mathcal{L}_{\vect\theta}[\rho_0,\vect\pi^{N+2}_{\vect\theta}]+V^{N+1}_{\vect\theta}[\rho^{\vect\pi^{N+2}_{\vect\theta}}_1]\nonumber\\&-\mathcal{L}_{\vect\theta}[\rho_0,\vect\pi^{N+1}_{\vect\theta}]-V^{N}_{\vect\theta}[\rho^{\vect\pi^{N+1}_{\vect\theta}}_1]
\end{align}
Then $\vect\pi^{N+1}_{\vect\theta}$ may not be optimal for the value function $V^{N+2}_{\vect\theta}[\rho_0]$ and \eqref{eq:pro1} reads as:
\begin{align}
    V^{N+2}_{\vect\theta}[\rho_0]&-V^{N+1}_{\vect\theta}[\rho_0]\leq \mathcal{L}_{\vect\theta}[\rho_0,\vect\pi^{N+1}_{\vect\theta}]+V^{N+1}_{\vect\theta}[\rho^{\vect\pi^{N+1}_{\vect\theta}}_1]\nonumber\\&-\mathcal{L}_{\vect\theta}[\rho_0,\vect\pi^{N+1}_{\vect\theta}]+V^{N}_{\vect\theta}[\rho^{\vect\pi^{N+1}_{\vect\theta}}_1]\leq 0
\end{align}
then by induction \eqref{eq:mono} holds $\forall N\in\mathbb{I}_{\geq 0}$.
\end{proof}

We next assume that the stage cost ${\mathcal{L}_{\vect\theta}}[\rho_0,\vect\pi]$, the terminal cost $T_{\vect\theta}$ and the terminal set $\Xi_{\mathrm{f}}$ satisfy the stabilizing conditions.
\begin{Assumption}\label{assum:LT}We assume that the stage cost satisfies:

and there exists a terminal policy $\vect\pi_{\mathrm{f}}$ such that the terminal cost $T_{\vect\theta}$ satisfies the following conditions, $\forall \rho_0\in\Xi_{\mathrm{f}}$:
\begin{subequations}
\begin{align}\label{eq:ter:assum}
    T_{\vect\theta}[\rho^{\vect\pi_{\mathrm{f}}}_{1}]-T_{\vect\theta}[\rho_{0}]&\leq-{\mathcal{L}_{\vect\theta}}[\rho_0,\vect\pi_{\mathrm{f}}]\\
\label{eq:ter2:assum}
    T_{\vect\theta}[\rho_0] &\geq 0\,\,,  
\end{align}
\end{subequations}
\end{Assumption}
Note that this assumption is a standard assumption for tracking MPC in order to show the closed-loop stability under the optimal policy resulting from the MPC-scheme. The terminal cost assumption can be satisfied using a generic non-negative functional approximator and designing a proper terminal set that contains the optimal steady-state measure $\rho^\star$. The stage cost assumption can be satisfied using constrained steps in the learning algorithm or providing a positive functional by construction. The details of these methods for deterministic systems can be found in \cite{Arash2021verification}. However, a detailed discussion on functional space is out of our scope.


